Demystifying Brain Tumour Segmentation Networks: Interpretability and Uncertainty Analysis

The accurate automatic segmentation of gliomas and its intra-tumoral structures is important not only for treatment planning but also for follow-up evaluations. Several methods based on 2D and 3D Deep Neural Networks (DNN) have been developed to segment brain tumors and to classify different categories of tumors from different MRI modalities. However, these networks are often black-box models and do not provide any evidence regarding the process they take to perform this task. Increasing transparency and interpretability of such deep learning techniques are necessary for the complete integration of such methods into medical practice. In this paper, we explore various techniques to explain the functional organization of brain tumor segmentation models and to extract visualizations of internal concepts to understand how these networks achieve highly accurate tumor segmentations. We use the BraTS 2018 dataset to train three different networks with standard architectures and outline similarities and differences in the process that these networks take to segment brain tumors. We show that brain tumor segmentation networks learn certain human-understandable disentangled concepts on a filter level. We also show that they take a top-down or hierarchical approach to localizing the different parts of the tumor. We then extract visualizations of some internal feature maps and also provide a measure of uncertainty with regards to the outputs of the models to give additional qualitative evidence about the predictions of these networks. We believe that the emergence of such human-understandable organization and concepts might aid in the acceptance and integration of such methods in medical diagnosis.

==> Interpretability and uncertainty analysis of DNN/frontiers_SupplementaryMaterial.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% This is just an example/guide for you to refer to when producing your supplementary material for your Frontiers article.                                 %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Version 2.5 Generated 2018/06/15 %%%
%%% You will need to have the following packages installed: datetime, fmtcount, etoolbox, fcprefix, which are normally inlcuded in WinEdt. %%%
%%% In http://www.ctan.org/ you can find the packages and how to install them, if necessary. %%%
%%%  NB logo1.jpg is required in the path in order to correctly compile front page header %%%

%\documentclass[utf8]{frontiers_suppmat} % for all articles

%\usepackage{hyperref}
\captionsetup[subfigure]{labelformat=empty}
%\usepackage{url,lineno,microtype}
%\usepackage[onehalfspacing]{setspace}
%\usepackage{amsmath}
\usepackage{subfig}
%\usepackage{graphicx}
\usepackage{float}
% \linenumbers
%\usepackage{nameref}

% Leave a blank line between paragraphs instead of using \\

%\begin{document}
% \onecolumn
% \firstpage{1}

% \title[Supplementary Material]{{\helveticaitalic{Supplementary Material}}}
\newpage

\section{Supplementary Material}

\subsection{Network Architectures}

\begin{figure}[H]
\centering
    \includegraphics[width=1.\textwidth]{networks.jpg}
    \caption{Network Architectures used in our study}
    \label{fig:fig8}
\end{figure}

\subsection{Network Dissection}


% \begin{figure}[H]
% \captionsetup[subfigure]{labelformat=empty}

% \centering
%   \subfloat[a]{\includegraphics[width=0.3\textwidth]{dense.png}}\hfill
%   \subfloat[b]{\includegraphics[width=0.3\textwidth]{resunet.png}}\hfill
%   \subfloat[c]{\includegraphics[width=0.3\textwidth]{simunet.png}}\\
%     \caption{Network Architectures used in our study}
%     \label{fig:fig5}
% \end{figure}

Final extracted disentangled concepts for different filters of a particular layer are shown. The figures clearly show that different filters are specialized to detect different concepts of the input image. All three networks show similar behaviour.

\begin{figure}[H]
\captionsetup[subfigure]{labelformat=empty}

    \centering
    {\includegraphics[width=0.9\textwidth]{sup_20_uresnet_conv2d_21_.jpg}}\hfill
    \caption{Concepts learned by filters of a particular layer of the ResUnet for an input image. (Conv Layer 21)}
\end{figure}

\begin{figure}[H]
\captionsetup[subfigure]{labelformat=empty}

    \centering
    {\includegraphics[width=0.9\textwidth]{sup_20_dense_conv2_block1_1_conv_.jpg}}\hfill
    \caption{Concepts learned by filters of a particular layer of the DenseUnet for an input image. (Encoding Block 1, Conv 2)}
\end{figure}

% \begin{figure}[H]
% \captionsetup[subfigure]{labelformat=empty}

%     \centering
%     {\includegraphics[width=0.9\textwidth]{sup_35_simnet_conv2d_21_.jpg}}\hfill
%     \caption{Concepts learned by filters of a particular layer of the SimUnet for an input image. (Conv Layer 21)}
% \end{figure}
\newpage

\begin{figure}[H]
\captionsetup[subfigure]{labelformat=empty}
\centering
   \subcaptionbox{(a)}{\includegraphics[width=0.4\textwidth]{grad_results_1.jpg}}\hfill
   \subcaptionbox{(b)}{\includegraphics[width=0.4\textwidth]{grad_results_2.jpg}}\\
    \caption{Grad-CAM results for consecutive layers of the ResUnet (view: top to bottom, column a, followed by top to bottom, column b)}
    \label{fig:fig12}
\end{figure}


\newpage
\subsection{Feature Visualization}

The figure below shows visualized features for a randomly selected filter of successive layers. 
\begin{figure}[H]
\captionsetup[subfigure]{labelformat=empty}

    \centering
    {\includegraphics[width=0.8\textwidth]{sup_hr.jpg}}\hfill 
    % \label{fig:fig11}
    \caption{Activation maps for layers of the ResUnet}
\end{figure}

\newpage
\begin{figure}[H]
\captionsetup[subfigure]{labelformat=empty}

    \centering
    {\includegraphics[width=0.95\textwidth]{regularizers.jpg}}\hfill 
    \label{fig:fig13}
    \caption{Effect of independently changing hyperparamaters for each regularizer. Top: Jitter coefficient increases [0 pixels, 1p, 6p, 12p, 20p], Middle: Style Coefficient increases [$10^{-2}$, $10^{-1}$, $1$, $5$, $10$], Bottom: Total Variation regularization increases [$10^{-7}$, $10^{-6}$, $10^{-5}$, $10^{-4}$, $10^{-3}$] to smoothen image}
\end{figure}

\subsection{Uncertainty}

\begin{figure}[H]
\captionsetup[subfigure]{labelformat=empty}
\centering
   {\includegraphics[width=0.9\textwidth]{sup_unc.jpg}}\hfill
    \caption{Uncertainty estimations (shown in red) for the DenseUnet (a,b,c,d) and ResUnet (e,f). Ground Truth(Left), Model Prediction(Middle), and Uncertainty(Right).}
    \label{fig:fig14}
\end{figure}
%\end{document}


==> frontiers_SupplementaryMaterial.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% This is just an example/guide for you to refer to when producing your supplementary material for your Frontiers article.                                 %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Version 2.5 Generated 2018/06/15 %%%
%%% You will need to have the following packages installed: datetime, fmtcount, etoolbox, fcprefix, which are normally inlcuded in WinEdt. %%%
%%% In http://www.ctan.org/ you can find the packages and how to install them, if necessary. %%%
%%%  NB logo1.jpg is required in the path in order to correctly compile front page header %%%

%\documentclass[utf8]{frontiers_suppmat} % for all articles

%\usepackage{hyperref}
\captionsetup[subfigure]{labelformat=empty}
%\usepackage{url,lineno,microtype}
%\usepackage[onehalfspacing]{setspace}
%\usepackage{amsmath}
\usepackage{subfig}
%\usepackage{graphicx}
\usepackage{float}
% \linenumbers
%\usepackage{nameref}

% Leave a blank line between paragraphs instead of using \\

%\begin{document}
% \onecolumn
% \firstpage{1}

% \title[Supplementary Material]{{\helveticaitalic{Supplementary Material}}}
\newpage

\section{Supplementary Material}

\subsection{Network Architectures}

\begin{figure}[H]
\centering
    \includegraphics[width=1.\textwidth]{networks.jpg}
    \caption{Network Architectures used in our study}
    \label{fig:fig8}
\end{figure}

\subsection{Network Dissection}


% \begin{figure}[H]
% \captionsetup[subfigure]{labelformat=empty}

% \centering
%   \subfloat[a]{\includegraphics[width=0.3\textwidth]{dense.png}}\hfill
%   \subfloat[b]{\includegraphics[width=0.3\textwidth]{resunet.png}}\hfill
%   \subfloat[c]{\includegraphics[width=0.3\textwidth]{simunet.png}}\\
%     \caption{Network Architectures used in our study}
%     \label{fig:fig5}
% \end{figure}

Final extracted disentangled concepts for different filters of a particular layer are shown. The figures clearly show that different filters are specialized to detect different concepts of the input image. All three networks show similar behaviour.

\begin{figure}[H]
\captionsetup[subfigure]{labelformat=empty}

    \centering
    {\includegraphics[width=0.9\textwidth]{sup_20_uresnet_conv2d_21_.jpg}}\hfill
    \caption{Concepts learned by filters of a particular layer of the ResUnet for an input image. (Conv Layer 21)}
\end{figure}

\begin{figure}[H]
\captionsetup[subfigure]{labelformat=empty}

    \centering
    {\includegraphics[width=0.9\textwidth]{sup_20_dense_conv2_block1_1_conv_.jpg}}\hfill
    \caption{Concepts learned by filters of a particular layer of the DenseUnet for an input image. (Encoding Block 1, Conv 2)}
\end{figure}

% \begin{figure}[H]
% \captionsetup[subfigure]{labelformat=empty}

%     \centering
%     {\includegraphics[width=0.9\textwidth]{sup_35_simnet_conv2d_21_.jpg}}\hfill
%     \caption{Concepts learned by filters of a particular layer of the SimUnet for an input image. (Conv Layer 21)}
% \end{figure}
\newpage

\begin{figure}[H]
\captionsetup[subfigure]{labelformat=empty}
\centering
   \subcaptionbox{(a)}{\includegraphics[width=0.4\textwidth]{grad_results_1.jpg}}\hfill
   \subcaptionbox{(b)}{\includegraphics[width=0.4\textwidth]{grad_results_2.jpg}}\\
    \caption{Grad-CAM results for consecutive layers of the ResUnet (view: top to bottom, column a, followed by top to bottom, column b)}
    \label{fig:fig12}
\end{figure}


\newpage
\subsection{Feature Visualization}

The figure below shows visualized features for a randomly selected filter of successive layers. 
\begin{figure}[H]
\captionsetup[subfigure]{labelformat=empty}

    \centering
    {\includegraphics[width=0.8\textwidth]{sup_hr.jpg}}\hfill 
    % \label{fig:fig11}
    \caption{Activation maps for layers of the ResUnet}
\end{figure}

\newpage
\begin{figure}[H]
\captionsetup[subfigure]{labelformat=empty}

    \centering
    {\includegraphics[width=0.95\textwidth]{regularizers.jpg}}\hfill 
    \label{fig:fig13}
    \caption{Effect of independently changing hyperparamaters for each regularizer. Top: Jitter coefficient increases [0 pixels, 1p, 6p, 12p, 20p], Middle: Style Coefficient increases [$10^{-2}$, $10^{-1}$, $1$, $5$, $10$], Bottom: Total Variation regularization increases [$10^{-7}$, $10^{-6}$, $10^{-5}$, $10^{-4}$, $10^{-3}$] to smoothen image}
\end{figure}

\subsection{Uncertainty}

\begin{figure}[H]
\captionsetup[subfigure]{labelformat=empty}
\centering
   {\includegraphics[width=0.9\textwidth]{sup_unc.jpg}}\hfill
    \caption{Uncertainty estimations (shown in red) for the DenseUnet (a,b,c,d) and ResUnet (e,f). Ground Truth(Left), Model Prediction(Middle), and Uncertainty(Right).}
    \label{fig:fig14}
\end{figure}
%\end{document}

